Why the World Reads Wikipedia: Beyond English Speakers

As one of the Web's primary multilingual knowledge sources, Wikipedia is read by millions of people across the globe every day. Despite this global readership, little is known about why users read Wikipedia's various language editions. To bridge this gap, we conduct a comparative study by combining a large-scale survey of Wikipedia readers across 14 language editions with a log-based analysis of user activity. We proceed in three steps. First, we analyze the survey results to compare the prevalence of Wikipedia use cases across languages, discovering commonalities, but also substantial differences, among Wikipedia languages with respect to their usage. Second, we match survey responses to the respondents' traces in Wikipedia's server logs to characterize behavioral patterns associated with specific use cases, finding that distinctive patterns consistently mark certain use cases across language editions. Third, we show that certain Wikipedia use cases are more common in countries with certain socio-economic characteristics; e.g., in-depth reading of Wikipedia articles is substantially more common in countries with a low Human Development Index. These findings advance our understanding of reader motivations and behaviors across Wikipedia languages and have implications for Wikipedia editors and developers of Wikipedia and other Web technologies.

==> sections/043corr_size.tex <==
\subsection{Survey responses and Wikipedia size}
\note{Why is talking about this section important? What do we learn by knowing about these relations? It's good to mention that at the beginning of this section for the reader to know why these can matter.}
\todo{If the decision is to keep this subsection, we can consider moving it to the end of the section and close the results with this. We want to share the most interesting results with the reader first, before we lose them. ;). Also, explain why only motivation is correlated with Wikipedia size as opposed to information depth and familiarity as well.}

To better understand the user intent for different Wikipedia editions, we correlate the survey responses with the sizes of Wikipedia editions as measured by the number of articles and by the number of pageviews received on the days of the survey. Since both measures are highly correlated (Spearman's $r_s=0.86$), we here present the results for pageviews only.

We observe that the prevalence of user motivations within a Wikipedia language correlates significantly with the number of pageviews in the language. In particular, we observe that motivations triggered by \emph{conversations} ($r_s=-0.78$, Bonferroni-corrected p-value $p=0.014$) or \emph{intrinsic learning} ($r_s=-0.78$, Bonferroni-corrected p-value ($r_s=-0.73, p=0.037$) are more common in the smaller Wikipedia languages. In these smaller languages, there is also a tendency towards using Wikipedia when motivated by \emph{personal decisions} ($r_s=-0.61$) or \emph{current events} ($r_s=0.54$).
On the other hand, larger Wikipedia editions are read more frequently by those that are motivated by \emph{media} ($r_s=0.56$) or are \emph{bored or randomly exploring Wikipedia} ($r_s=0.54)$.

==> sections/obs_041vs2016.tex <==
%%%%%
% CURRENTLY NOT INCLUDED
%%%%%

\subsection{Comparison with 2016 results.}
\note{Consider shortening this section significantly if short in space. We can drop the section altogether and add a few sentences to say the result.}
%consider shortening it significantly if short in space



In order to assess the stability of our survey results, we start by comparing the results for the English Wikipedia with the previous study of March 2016\cite{singer2017we}. 
We can observe that overall the survey results are very similar, see Figure~\ref{fig:2016 vs 2017}.
For all user motivations with the exception of \emph{work/school} are within two percentage points of the results of the previous study.
For \emph{work/school}, we see a significant decrease from around 16\% to around 10\%. 
A potential explanation for this might the different season of year (March vs June) the surveys took place, which might have lead to more workers on holiday or less students in exam preparation in 2017.
Also regarding information depth and prior knowledge are fully in line with the 2016 results. 
%The need for fact checking and overview are on about the same level, while in-depth reading is less often intended. 
We only observe a slight increase of in-depth reading from 21.9\% to 26.0\% percent.
%The prior knowledge of the topic remains stable at about 50\% for both answer option, i.e. "familiar" and "unfamiliar"

==> sections/readersPerCountry.tex <==
\subsection{Readers across Countries and Languages}


\begin{figure*}[t]
\centering
\includegraphics[width=0.95\textwidth]{results/bigestShareofPageViewsPerCountry.png}
\label{fig:shareOfPageViews}  
\end{figure*}


Giving that the English Wikipedia is at least 4 times bigger than the following one, it is important to understand
 the relevance of having content in written in a given language, depending on the country were that content is being read.


Not surprising, figure \ref{fig:shareOfPageViews} shows that most of the countries have a clear dominant project, corresponding to the predominant language in that country. Exceptional cases like Belgium or Switzerland (CH), can be explained by the fact those countries have language diversity within their borders.
However, by increasing the geographical  granularity of our analysis, we see that in each region of Belgium there is clear dominant project (see Table \ref{table:belgium}). As consequence of the previous results, we found  that  in non-English speaking countries, the number of people visiting the English Wikipedia is marginal (less than 20\%) reinforcing the the relevance of  content in  local languages.

\begin{table}
\caption{\emph{Projects Views within Belgium:} Here we show the 3 top projects visited per region in Belgium, the country with largest diversity of projects views in our sample. This results shows that the idea of diversity of languages in Belgium is an artefact of geographical granularity. We found similar results for Switzerland.}
\label{table:belgium}
\begin{tabular}{llc}
\toprule
Region &       Project &  Share of Pageviews \\
\midrule
Brussels Capital &  fr.wikipedia &   45$$\%$$   \\
 &  en.wikipedia &   33$$\%$$   \\
 &  nl.wikipedia &   11$$\%$$   \\
 & others & 11$$\%$$  \\
\midrule 

Flanders    &  nl.wikipedia &   54$$\%$$  \\
    &  en.wikipedia &   36$$\%$$  \\
   &  fr.wikipedia &    5$$\%$$  \\
   & others & 5 \\
 \midrule
Wallonia    &  fr.wikipedia &   75$$\%$$  \\
    &  en.wikipedia &   17$$\%$$  \\
    &  nl.wikipedia &    3$$\%$$  \\
        & others&    5$$\%$$  \\
\bottomrule
\end{tabular}
\end{table}


